Do Unit Proofs Work? An Empirical Study of Compositional Bounded Model Checking for Memory Safety Verification

Memory safety defects pose a major threat to software reliability, enabling cyberattacks, outages, and crashes. To mitigate these risks, organizations adopt Compositional Bounded Model Checking (BMC), using unit proofs to formally verify memory safety. However, methods for creating unit proofs vary across organizations and are inconsistent within the same project, leading to errors and missed defects. In addition, unit proofing remains understudied, with no systematic development methods or empirical evaluations. This work presents the first empirical study on unit proofing for memory safety verification. We introduce a systematic method for creating unit proofs that leverages verification feedback and objective criteria. Using this approach, we develop 73 unit proofs for four embedded operating systems and evaluate their effectiveness, characteristics, cost, and generalizability. Our results show unit proofs are cost-effective, detecting 74\% of recreated defects, with an additional 9\% found with increased BMC bounds, and 19 new defects exposed. We also found that embedded software requires small unit proofs, which can be developed in 87 minutes and executed in 61 minutes on average. These findings provide practical guidance for engineers and empirical data to inform tooling design.

==> misc/realistic-program.tex <==
\begin{listing}
        % \centering
        \begin{minted}[
            fontsize=\scriptsize,
            linenos,
            gobble=2, % Remove unnecessary indentation -- the line numbers make this clear enough
            xleftmargin=0.5cm, % Otherwise we start in the left margin...
            escapeinside=||, % Allows you to use LaTeX commands inside code
            style=colorful,   % You can change this to another style like 'monokai', 'borland', etc.
            breaklines        % Break long lines
        ]{c}

void processReceivedData(uint8_t *data, uint16_t len, uint16_t offset) {
    ...
    CurrentCtx *ctx = getCurrentCtx();
    ...
    memcpy(ctx->payload + offset, data, len)
}

        \end{minted}

        \caption{A simple systematically-developed unit proof.
        } % Optional caption
        \label{code:simple-program}
\end{listing}

==> misc/realistic-proof.tex <==
\begin{listing}
        % \centering
        \begin{minted}[
            fontsize=\scriptsize,
            linenos,
            gobble=2, % Remove unnecessary indentation -- the line numbers make this clear enough
            xleftmargin=0.5cm, % Otherwise we start in the left margin...
            escapeinside=||, % Allows you to use LaTeX commands inside code
            style=colorful,   % You can change this to another style like 'monokai', 'borland', etc.
            breaklines        % Break long lines
        ]{c}

// Function models
TCPHeader * type1Model() |\dingrone| {
    TCPHeader *header = malloc(sizeof(TCPHeader));
    return header;
}

TCPHeader * type2Model(TCPHeader *header, uint16_t headerLen) |\dingrtwo| {
    uint8_t offset;
    __CPROVER_assume(offset < headerLen); |\dingfive|
    return header + offset;
}

void type3Model(unit8_t **ptr, uint8_t *ptrSize) |\dingrthree| {
    uint8_t size; *ptr = malloc(size);
    _assume(ptr != NULL); |\dingone|
    *ptrSize = size;
}

extern uint16_t uip_ext_len; extern uint16_t uip_len;

// Loop bounds
_unwind(funcUnitEntryPoint.0:4);
_unwind(funcUnitEntryPoint.0:2);

void unitProof () {

    int dataLength;
    uint8_t *data = malloc(dataLength);
    uint8_t type;
    uint8_t numOptions;

    buf->handler = type1Model;

    // Variable models
    __CPROVER_assume(dataLength > sizeof(TCPHeader)); |\dingthree|
    if (type == TYPE_DIRECT_IND) { |\dingsix|
        __CPROVER_assume(numOptions < 4); |\dingfour|
    } else {
        __CPROVER_assume(numOptions < 16); |\dingfour|
    }
    __CPROVER_assume(uip_ext_len < uip_len); |\dingfive|

    funcUnitEntryPoint(data, dataLength, numOptions); |\dingfive|
}

        \end{minted}

        \caption{A systematically-developed unit proof. % showing modeled input variables, global variables and functions. 
        For realism, each element is taken from a real proof.
        In step 1, the initial unit proof contained only the black box. 
        Initial verification timed out due to an unconstrained function pointer.
        In step 2, we resolved this (adding red box).
        The coverage report showed gaps due to insufficient loops.
        In step 3, we increased the bounds of affected loops (adding green box).
        Finally, the error report indicated errors caused by unknown variables and functions.
        In step 4, we resolved these via variable preconditions (blue box) and function models (orange box).
        } % Optional caption
        \label{code:realistic-unit-proof}
\end{listing}

==> misc/simple-realistic-proof.tex <==
\begin{listing}
        % \centering
        \begin{minted}[
            fontsize=\scriptsize,
            linenos,
            gobble=2, % Remove unnecessary indentation -- the line numbers make this clear enough
            xleftmargin=0.5cm, % Otherwise we start in the left margin...
            escapeinside=||, % Allows you to use LaTeX commands inside code
            style=colorful,   % You can change this to another style like 'monokai', 'borland', etc.
            breaklines        % Break long lines
        ]{c}

// Function model
CurrentCtx *getCurrentCtx(){
    CurrentCtx *ctx = malloc(sizeof(CurrentCtx));
    return ctx;
}

extern uint16_t uip_ext_len; extern uint16_t uip_len;

void harness () {

    uint16_t dataLength;
    uint16_t offset;
    uint8_t *data = malloc(dataLength);

    // Input variable models
    __CPROVER_assume(dataLength > sizeof(TCPHeader)); 
    __CPROVER_assume(data != NULL);
    __CPROVER_assume(offset < dataLength);

    // Global variable models
    __CPROVER_assume(uip_ext_len < uip_len);

    processReceivedData(data, dataLength, offset); 
}

        \end{minted}

        \caption{A simple systematically-developed unit proof.
        } % Optional caption
        \label{code:simple-unit-proof}
\end{listing}
